Adversarial Inverse Graphics Networks: Learning 2D-to-3D Lifting and Image-to-Image Translation from Unpaired Supervision

Researchers have developed excellent feed-forward models that learn to map images to desired outputs, such as to the images' latent factors, or to other images, using supervised learning. Learning such mappings from unlabelled data, or improving upon supervised models by exploiting unlabelled data, remains elusive. We argue that there are two important parts to learning without annotations: (i) matching the predictions to the input observations, and (ii) matching the predictions to known priors. We propose Adversarial Inverse Graphics networks (AIGNs): weakly supervised neural network models that combine feedback from rendering their predictions, with distribution matching between their predictions and a collection of ground-truth factors. We apply AIGNs to 3D human pose estimation and 3D structure and egomotion estimation, and outperform models supervised by only paired annotations. We further apply AIGNs to facial image transformation using super-resolution and inpainting renderers, while deliberately adding biases in the ground-truth datasets. Our model seamlessly incorporates such biases, rendering input faces towards young, old, feminine, masculine or Tom Cruise-like equivalents (depending on the chosen bias), or adding lip and nose augmentations while inpainting concealed lips and noses.

==> abstract_old.tex <==
\begin{abstract}
  We introduce a neural network that learns to map images or image pairs to latent factors, \eg, 3D object poses, 3D geometry of the scene and camera viewpoints, using two forms of weak supervision.
  First, 
  
  The first form of supervision is a reconstruction loss: the predicted latent factors are rendered into an image, and a loss is generated if the render differs from the original input. The second is a distribution matching loss on the latent factors: the predicted factors are compared against ground truth ones by an adversarial network, and a loss is generated if the predicted factors deviate from the ground truth distribution. The reconstruction loss ensures that the predictions are tailored to the input, while the distribution matching loss ensures that the predictions are plausible. Applied together, these losses demand that the network learn inverse graphics.
  
  We apply this approach to 3D human pose estimation and 3D structure and egomotion estimation, and outperform models supervised by paired annotations and reconstruction losses. We additionally perform experiments with super-resolution and inpainting tasks, and find that the model is surprisingly effective at ``visual plastic surgery''. If one designs a ground truth set that contains a strong bias, for instance towards ``young'' faces, the super-resolution process makes the face appear younger. Similarly, one can create an intentional bias in the inpainting network, such that it creates lip or nose augmentations while inpainting concealed lips and noses.
\end{abstract}


\begin{abstract}
  We introduce a neural network that learns to generate the latent factors of images (\eg, poses of humans, 3D geometry of the scene), by two forms of weak supervision. The first form of supervision is a reconstruction loss: the predicted latent factors are rendered into an image, and a loss is generated if the render differs from the original input. The second is a distribution matching loss on the latent factors: the predicted factors are compared against ground truth ones by an adversarial network, and a loss is generated if the predicted factors deviate from the ground truth distribution. The reconstruction loss ensures that the predictions are tailored to the input, while the distribution matching loss ensures that the predictions are plausible. Applied together, these losses demand that the network learn inverse graphics.
  
  We apply this approach to 3D human pose estimation and 3D structure and egomotion estimation, and outperform models supervised by paired annotations and reconstruction losses. We additionally perform experiments with super-resolution and inpainting tasks, and find that the model is surprisingly effective at ``visual plastic surgery''. If one designs a ground truth set that contains a strong bias, for instance towards ``young'' faces, the super-resolution process makes the face appear younger. Similarly, one can create an intentional bias in the inpainting network, such that it creates lip or nose augmentations while inpainting concealed lips and noses.
\end{abstract}

Researchers have developed excellent feed-forward models that learn to map images to desired output, -\eg,  latent factors or image transformations- using supervised learning. Learning such mapping from unlabelled data or improving upon  supervised models by exploiting unlabelled data still remains elusive. 
We argue that there are two important components in learning without annotations: (1) whether the predictions match the input observations and (2) prior or bias about what to predict. We propose Adversarial Inverse Graphics networks (AIGNs), weakly supervised neural network models that combine feedback from rendering their predictions, as well as distribution matching between their predictions and a set of a collection of ground-truth factors, unrelated (unpaired) to  the current input. 
Our model can thus be self-supervised by unlabelled image data, by minimizing a joint reconstruction and adversarial loss, complementing any direct supervision provided by paired annotations. 

% fish poster abstract
% Researchers have developed excellent feed-forward models that learn to map images to desired outputs (ex. edited images or 3D predictions) using supervised learning. However, certain annotations are very hard or not possible to obtain (ex. images of male and the corresponding images of turning them into women). Besides, from biological point of view, we as human often learn without labels. In this work, we exploit a way to leverage unlabelled data. We argue that there are two important components in learning without annotations: (1) whether the prediction matches with what we observe and (2) bias about what to predict. We propose adversarial inversion, a weakly supervised neural network model that combines feedback from rendering its predictions, as well as distribution matching between its predictions and a set of stored examples.

%We argue that there are two important components in learning without annotations: (1) whether the prediction matches the observations, and (2) 
%about what to predict.
%Unsupervised learning methods are critical for tasks
%In tasks that require extensive human labelling effort, such as 
%unsupervised learning is key.
%There are many tasks for which it takes significant human effort to create labels.
%extensive human effort to create labels.
%Unsupervised learning is critical for any task that requires 
%Supervised learning has yielded excellent feed-foward models for some tasks (\eg, object detection, or semantic segmentation),
%to create labels, such as Photoshopping a given person to look younger, 
%\eg, human pose annotation, or realistic Photoshopping
% Supervised learning has brought
%There exist excellent feed-forward models that
%map images to a variety of desirable outputs using supervised learning (\eg, object detection, or semantic segmentation). However, many desirable outputs require extensive human labelling effort, \eg, human pose annotation, or realistic Photoshopping. This work presents a way to learn such tasks with unlabelled data. We 
%two important components in learning without annotations: (1) whether the prediction matches with what we observe and (2) bias about what to predict. We propose adversarial inversion, a weakly supervised neural network model that combines feedback from rendering its predictions, as well as distribution matching between its predictions and a set of stored examples.



==> related.tex <==
\section{Related Work}
\begin{comment}
\paragraph{Priors}

Many approaches on inverse problems (\eg, 3D human pose estimation, structure from motion, intrinsic image decomposition \etc.) do not learn to map visual input to desired predictions, but rather rely on optimization and hand designed priors, such as sparsity in \cite{Yang:2010:ISV:1892456.1892463}, spatial smoothness (for optical flow, depth, albedo, etc.), temporal smoothness for shading in \cite{Kong:ECCV:2014} or motion in \cite{Yang:2010:ISV:1892456.1892463}, low-rank 3D shape or trajectory priors in \cite{Sheikh_2008_6196,Wu2016}, deformable 3D scene models in  \cite{PICTURE,DBLP:journals/corr/AlldieckKM17}, and many others. Hand designed priors generalize well but they are often too generic. AIGNs instead uses data driven priors through distribution matching between predictions and (unpaired) ground-truth memories.  Adversarial  priors exploit  unlabelled data available in the form of  latent factor repositories, e.g., collections of human 3D poses, collections of egomotions of a self-driving car etc.,  which lie in a thin manifold over the whole space of 3D keypoints or 3D rotations and translations, respectively. In this way,  predictions are regularized.
\end{comment}


\noindent
\textbf{Conditional image generation}
Conditional Generative Adversarial Networks sample (or deterministically predict)  images   conditioned on visual input, where jointly trained discriminator networks provide feedback on how well the image samples match real images \cite{NIPS2014_5423}. Previous conditional GAN formulations  \cite{DBLP:journals/corr/MirzaO14,DBLP:journals/corr/IsolaZZE16} need paired annotations for supervision (a dataset where each input image is paired with the corresponding desired output). 
 %This is necessary, since otherwise we cannot ensure that correct predictions will be generated.  % thus distribution matching takes places between the predicted images and 

AIGNs extend  conditional GAN formulations in two ways: first, using feedback in the form of reconstruction accuracy  between rendered predictions and original input.  Such feedback loop permits using \textit{unpaired} annotations for the discriminators, in a looser but  unsupervised  distribution matching.  
%GAN formulations -concurrent works of \todo{cite} \cite{} also show lie on the unpaired domain- and demonstrate them as a way  to impose general data-driven priors, 
Second, it uses distribution matching over latent factors as opposed to image domains, e.g., on 3D human poses and camera frame-to-frame 3D rotations and translations. 
AIGNs are also related to  adversarial autoencoders \cite{DBLP:journals/corr/MakhzaniSJG15}. In AIGNs,  latent intermediate variables represent not Gaussian distributions but rather interpretable visual quantities, and parametric decoders of autoencoders are replaced by  parameter-free renderers.  

 

Work of Attribute2image \cite{DBLP:journals/corr/YanYSL15} is a variational autoencoder model that given an input image and a desired attribute vector generates images that have those attributes, e.g., ``old", ``male", ``brown hair" \etc. It is trained with   strong supervision, where each training image is annotated with a set of attributes.  Attribute "progression" ( \eg changing male to female) is achieved by varying the value of the target attribute in the input vector. In the experimental section, we compare our model against Attribute2Image and show our result  better preserves the fidelity of the transformation  and  has  higher level of detail, at the negligible cost of training a different super-resolution or inpainting model for each desired transformation. Further, our transformations can reflect \textbf{fine-grained visual attributes} described by a set of exemplar images (as discriminator memories), as opposed to 
%e.g., we can transform a face to be more like Tom Cruise  or have  Michael Jackson nose.  This is not possible with previous supervised models whose transformations are described by 
coarse attribute  categories, e.g., ``old". 
%we can regulate how old or feminine some  described by few  is regulated by managing image memories not be textual attributes  which is much more expressive than just assigning attributes.





\noindent
\textbf{3D human pose estimation}
Recent works use deep neural networks and large supervised training sets \cite{h36m_pami} and learn to regress to 3D poses directly, given an RGB image \cite{DBLP:journals/corr/PavlakosZDD16}. Many have explored 2D body pose as an intermediate representation \cite{DBLP:journals/corr/ChenR16a,Wu2016,DBLP:journals/corr/TomeRA17}, or as an  auxiliary task in a multi-task setting \cite{DBLP:journals/corr/TomeRA17} where the abundance of labelled 2D pose training examples  helps feature learning and complements limited 3D supervision.  

\begin{comment}
Few have considered massive photorealistic data augmentation by rendering synthetic people against realistic backgrounds  \cite{DBLP:journals/corr/RogezS16} to obtain diverse RGB to 3D pose synthetic annotations, since  3D supervision requires a Vicon system and thus constrained setups. 
\end{comment}

%Work of 3d interpreter \cite{Wu2016}, same as our work, estimates both 3d pose and camera parameters and considers a 2d reprojection loss  to exploit training data with annotated 2d but not  3d information. Our work similarly targets weak supervision and explores  adversarial 3d human shape priors to complement 2d reprojection error of \cite{Wu2016}. We  show empirically our adversarial inversion model outperforms \cite{Wu2016} suggesting that adversarial priors are worthwhile and outperform previously employed   low-rank 3d shape priors \cite{Wu2016} or sparse priors  \cite{DBLP:journals/corr/ZhouZPLDD17}. % \todo{+?}.



\noindent
\textbf{Structure-from-motion/SLAM}
Simultaneous Localization And Mapping (SLAM) geometric methods have shown impressive results on estimating camera pose and 3D point clouds from monocular, stereo, or RGB-D video sequences \cite{schoeps14ismar,kerl13iros} using alternate optimization over camera poses and the 3D scene pointcloud. 
There has been a recent interest in integrating learning to aid  geometric approaches handle moving objects and low-texture image regions. The work of Handa et al. \cite{handa2016gvnn} contributed a  deep learning library with many geometric operations including a differentiable camera projection layer, similar to those used in SfM networks \cite{sfmnet,tinghuisfm}, 3D image interpreters \cite{interpreter}, and  depth from stereo  CNN~\cite{garg2016unsupervised}. Our Structure-from-motion AIGN architecture build upon those works. 

\begin{comment}

\paragraph{Super-resolution - Inpainting}
Deep neural network architectures have recently shown excellent performance on the task of super-resolution \cite{DBLP:journals/corr/DongLHT15,DBLP:journals/corr/BrunaSL15} and non-blind inpainting \cite{pathakCVPR16context,DBLP:journals/corr/YehCLHD16} (inpainting where the mask is always at the same part of the image). Adversarial losses have been used to resolve the regression to the mean problem of standard $L_2$ loss \cite{DBLP:journals/corr/LedigTHCATTWS16,pathakCVPR16context}. 
Our model unifies 
recent works of \cite{sonderby2014apparent} and \cite{DBLP:journals/corr/YehCLHD16} that combine adversarial and reconstruction losses for super-resolution and inpainting respectively, without paired supervision, same as our model. 
However, weak (unpaired) supervision might be unnecessary for  super-resolution or inpainting  as an unlimited amount of ground-truth pairs can be easily collected by downsampling or masking images. Our AIGN focuses instead on \textit{biased} super-resolution and  inpainting, as a tool towards creative and controllable image generation. 
\end{comment}

